Momentum Posterior Regularization for Multi-hop Dense Retrieval

Multi-hop question answering (QA) often requires sequential retrieval (multi-hop retrieval), where each hop retrieves missing knowledge based on information from previous hops. To facilitate more effective retrieval, we aim to distill knowledge from a posterior retrieval, which has access to posterior information like an answer, into a prior retrieval used during inference when such information is unavailable. Unfortunately, current methods for knowledge distillation in one-time retrieval are ineffective for multi-hop QA due to two issues: 1) Posterior information is often defined as the response (i.e. the answer), which may not clearly connect to the query without intermediate retrieval; and 2) The large knowledge gap between prior and posterior retrievals makes existing distillation methods unstable, even resulting in performance loss. As such, we propose MoPo (Momentum Posterior Regularization) with two key innovations: 1) Posterior information of one hop is defined as a query-focus summary from the golden knowledge of the previous and current hops; 2) We develop an effective training strategy where the posterior retrieval is updated along with the prior retrieval via momentum moving average method, allowing smoother and effective distillation. Experiments on HotpotQA and StrategyQA demonstrate that MoPo outperforms existing baselines in both retrieval and downstream QA tasks.

==> figs/posterior_motivation.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{lccc}
        \toprule
        Format & MDR & PR & MoPo\\
        \midrule
        Original Query  & 90.44 & 80.67 & 94.67 \\
        
        Full Answer   & 92.32 & 84.58 & 96.35 \\
        \bottomrule
    \end{tabular}
    \caption{Retrieval performance in Recall@100 on Hot-
potQA using 1st hop golden summary with different query format}
    \label{tab:posterior_motivation}
\end{table}

==> figs/raw_model_testing.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{lcc}
        \toprule
         & 1st hop & 2nd hop \\
        \midrule
        \textit{w/} Posterior Information  & 88.63 & 85.37  \\
        
        \textit{w/o} Posterior Information   & 83.21 & 81.84  \\
        \bottomrule
    \end{tabular}
    \caption{Zero-shot retrieval performance in Recall@100 with and without posterior information on 1350 HotpotQA dev samples. More experimental details are in Appendix \ref{section:raw_model}. }
    %\todo{ncamtu: C1 does not show any comparison between with or without posterior information. If you use golden posterior information for these results, then it is redundant. Of course, golden PI is helpful, there is no argument over that. Wuyuyang: Here we choose using this experiment to prove our guess: goldenPI is helpful}
    \label{tab:raw_model}
\end{table}

==> figs/structure.tex <==
\begin{figure*}
  %\includegraphics[width=\columnwidth]{figures/structure.eps}
  \includegraphics[width=\columnwidth]{example-image-duck}
  \includegraphics[width=\columnwidth]{example-image-duck}
  %\caption{Schematic diagram of multi-hop paragraph retrieval process using summary model to reconstruct query}
  \caption{I'm a little duck, quack quack quack quack quack quack quack quack quack quack quack quack quack quack quack quack quack quack }
  \label{fig:structure}
\end{figure*}
